The Enemy Within: The Emerging Threats to Healthcare from Malicious Mobile Devices

With the proliferation of wireless networks, mobile devices and medical devices are increasingly being equipped with wireless interfaces, such as Bluetooth and WiFi to allow easy access to and control of the medical devices. Unfortunately, the very presence and usage of such interfaces also expose the medical devices to novel attacks from malicious parties. The emerging threat from malicious mobile devices is significant and severe, since attackers can steal confidential data from a patient's medical device. Also, attackers can compromise the medical device and either feed doctors bad data from it or issue potentially fatal commands to the device, which may even result in the death of the patient. As the mobile devices are often at close proximity to the patient (either in the hospital or home settings), attacks from such devices are hard to prevent. In this paper, we present a systematic analysis of this new threat from mobile devices on medical devices and healthcare infrastructure. We also perform a thorough security analysis of a major hospital and uncover potential vulnerabilities. Finally, we propose a set of potential solutions and defenses against such attacks.

==> casestudy.tex <==
\section{Case Study}
\label{sec:casestudy}
To explore the current security state of typical medical devices used in hospitals, we analyzed  the system of a large university healthcare facility. Our tests found several vulnerabilities in the ongoing usage model for medical devices.\\

\noindent\textbf{Current Security Measures:~} We found two security measures taken by the medical. Firstly, to avoid any intrusion in WiFi network of medical devices, the hospital maintains a separate WiFi network for medical devices and users. Patient or medical personnel can not use this WiFi network, dedicated for medical devices. And secondly, to ensure the data security, for some medical devices, Secured Socket Layer (SSL) is used to communicate with the central patient monitoring or EMR management system. \\

\noindent\textbf{Vulnerabilities and Possible Attack Scenarios:~}
Separate WiFi network for medical devices and smart mobile devices can secure the system against integrity violation, but still it is possible to attack on privacy and availability. Also, for personal health monitoring devices used at a home or workplace setting outside healthcare facilities, this precaution will be invalid since users need to connect their mobile devices with the medical devices via their home or work networks to observe their health condition. Even in the hospital,  we were able to sniff the packets without connecting to the WiFi network. From the broadcast packets, we got the MAC and IP address of the surrounding devices and the wireless access points. By masquerading the IP address, it is possible to launch a DoS attack. The MAC address can also be used to identify device types and thereby infer the patient's confidential illness.

We identified insecurity in general purpose pumping machines, which communicate with the central patient monitoring system over the SSL through a gateway. They convey patientsÕ health condition to the central monitoring system, which returns appropriate dose of medicine to the pumping machines. Though it is not possible to intrude into a SSL communication, it is still prone to DoS attacks. Also, the gateway IP address was hard-coded in the device and was detected by our packet sniffer. Jamming this IP is possible which will make the communication channel unavailable. We cannot prevent this  without updating the firmware as the gateway IP address is not configurable.

We also explored the vulnerabilities of medical devices, which use WiFi but do not communicate over SSL. One such machine is vital sign (body temperature, pulse rate or heart rate, blood pressure, and respiratory rate) monitor system. It communicates with the central EMR system over WiFi, without using SSL, even though it carries sensitive health information and Nurse's login credentials. Nurses need to login to this device to send information to the EMR system. As we were able to get the Address Resolution Protocol (ARP) packets from the channel, we could potentially launch a MITM attack by ARP spoofing to get all the data packets sent for the EMR system \cite{website:ettercap}. That device supports both Wired Equivalent Privacy (WEP) and WiFi Protected Access 2 (WPA2) encryption scheme. We can compromise the WEP encryption and get the actual EMR from this channel \cite{Stubblefield01usingthe}. Using some tools, such as Aircrack \cite{website:aircrack}, one can also learn about the patients' EMR. Nurse's login credentials can be exposed in the same way, which will be extremely dangerous for the whole EMR management system, since the adversary can gather anyone's confidential medical data by posing as a nurse.

Our brief analysis confirms our original arguments regarding the safety of WiFi and Bluetooth enabled medical devices. The vulnerabilities we exposed show that such devices are prone to different types of attacks from mobile malware.\\

==> conclusion.tex <==
\section{Conclusion and Future Work}
\label{sec:conclusion}
As mobile devices become smarter, the threats from mobile malware to surrounding infrastructure also increases. WiFi and Bluetooth interfaces enable seamless communication between medical devices and other parts of the healthcare infrastructure. However, this capability has increased the attack surface of medical devices and opens the possibility of novel attacks. We argue that threats on medical devices from mobile devices, especially malware based attacks, are still unexplored, though mobile malware is exploding. 

In this paper, we explored the threat of attacks from mobile devices to medical devices. We posit that the intrinsic nature of mobile computing makes the problem difficult: mobile devices are likely to be inside the security perimeter of the healthcare facility's network, be close to the patient, and can be used to launch localized attacks. We also opine that the resource limitation in both medical and mobile devices is one of the main obstacles to defend against these attacks. To protect vital medical devices from attacks, we need to explore the problem domain deeply and develop effective and low-cost solutions.  In future research, our goal is to build a proof-of-concept application on Android platform which can be used to evaluate a medical network for vulnerabilities. We also plan to build and test our network anomaly based intrusion detection scheme to detect attacks on medical devices.\\    


==> motivation.tex <==
\section{Motivation and Threat Model}
\label{sec:motivation}
In this section, we present our motivation for exploring possible threats from smart mobile devices to new generation Bluetooth or WiFi-enabled medical devices. We also discuss the threat model.\\

\subsection{Motivation}
While mobile malware and attacks on medical devices are not new phenomena, the combination of these two things can be devastating. Availability of WiFi and Bluetooth has made mobile devices more powerful than they ever were. However, at the same time, this has also increased the risks of new ways of attacks. Botnet command-and-control networks have used Bluetooth as a communication medium \cite{singh2010evaluating}. Android phones can also be used to exploit Bluetooth interface to hack into a car's Electronic Control Unit \cite{checkoway2011comprehensive}. A lot of other attacks from smart phones are stated by Guo et al. \cite{guo2004smart}. Medical devices are also not safe from various kinds of attacks. It is possible to launch a software radio attack on implantable cardiac defibrillators and pacemakers \cite{halperin2008pacemakers}. Devices, such as, insulin pumps and glucose meters have also been successfully hacked \cite{bloomberg2012jackinsulin,mhhs2011jeromeinsulinpump}. 

As both smart mobile devices and medical devices are now equipped with Bluetooth and WiFi interfaces, attackers can launch attacks on medical devices from compromised mobile devices. The consequence of such attacks on medical devices ranges from threats to the patientÕs reputation to even her life. Sniffing EMR from the communication channels can be highly attractive to attackers because of the business value of medical records. Some attacks, such as providing wrong information to display devices or sending malicious command to some Implantable Medical Devices (IMD) or wearable devices, can actually place the patient's life in jeopardy. Murderers can use this as their killing tool as it is quite impossible to investigate \cite{goodman2011does}. Moreover, mobile malware based attack can open the opportunity of launching localized attacks. For example, adversary can target the topmost employees of an organization and if they wear any WiFi Real Time Location Service (RTLS) enabled device, she can monitor their location continuously. Therefore, it is important to systematically analyze the threats to medical devices from smart mobile devices and develop mitigation strategies.\\

\subsection{Threat Model}
To illustrate our threat model, we rely on the \emph{Bring Your Own Device} (BYOD) model \cite{bcs2011mobile}. This model has attracted the attention of corporate security researchers exploring the enterprise security problem space \cite{barr2010vmware}. Modern office managers let their employers bring their own smart devices, such as, laptop, smart phone, tablet, etc.. The downside is that, an infected tablet or smart phone belonging to an executive can easily enter the system and the malware may thus be running inside the security perimeter of the corporation. In a healthcare setting, this will involve a mobile device belonging to a doctor, patient or a visitor who is present inside a healthcare facility or a person's house. Even if the patient is using strong security for her computing infrastructure, the infected device will likely be in the vicinity of the medical device. We assume that these mobile devices  have already been infected by malware. This is possible when users download an untrusted application from the application store \cite{felt2011survey}. It is also possible to embed a malware in a trusted application or push a malware through an update patch of an existing application.

Pairing mechanism in Bluetooth channel offers most of the security of this channel. We assume that the malware affected devices are already paired with the Bluetooth-enabled medical device. This assumption is fairly common in malware research since people usually have many of their own mobile devices paired for their convenience. For example, while hacking a car's control unit, Checkoway et al. used an Android phone which was already paired with the car \cite{checkoway2011comprehensive}. In the medical environment, this is more likely, where mobile devices belonging to healthcare personnel and/or patients are usually paired with the medical devices for their own interest (for example, a mobile bloodpressure app paired with a wearable blood pressure monitor). This assumption is sufficient to launch a Denial of Service (DoS) attack. We also assume that the attacker is capable of reverse engineering the application protocol of the Bluetooth-enabled medical devices. This can make her capable of learning patient data as well as sending incorrect signal to medical devices.

To attack through the WiFi channel, we assume that the malware infected mobile devices are already connected to the access point and the attacker can reverse engineer the application protocol. These assumptions are sufficient for DoS attack and to interfere the communication between mobile devices and WiFi-enabled medical devices.\\

==> relatedwork.tex <==
\section{Related Work}
\label{sec:relatedwork}

Many researchers have explored the vulnerability of wireless-enabled medical devices. Halperin et al. presented a software radio attack on pacemakers and implantable cardiac defibrillators (ICD) \cite{halperin2008pacemakers}. The ICD was designed to communicate in 175 kHz frequency with an external application. They reverse engineered the ICD's protocols to launch attacks on integrity and confidentiality of data. They showed that the communication channel was unencrypted, and it is possible to change the operation of the ICD. They also proved that a battery-powered ICD can be kept busy continuously by an unauthenticated device, which can eventually drain out the battery power.

Radcliffe successfully hacked his own insulin pump \cite{mhhs2011jeromeinsulinpump}. He showed that untraceable attacks against wireless insulin pumps, pacemakers and ICDs are possible from half a mile away. As the transmissions were not encrypted, he was able to decipher the messages. He successfully reverse engineered the application protocol. At first, he successfully jammed the communication channel. Later, he gained full control over the insulin pump and glucose meter. Researchers at McAfee Inc. also successfully compromised an insulin pump \cite{bloomberg2012jackinsulin}, and were able to find vulnerable insulin pumps and send lethal doses from a distance of 300 feet.

These attacks were done by reverse engineering the radio channel, without any direct knowledge of the proprietary communication protocol. New generation medical devices communicate over Bluetooth or WiFi channels. The protocol standard of these technologies is open to everyone. Also, Denial of Service attacks or packet sniffing do not require any reverse engineering, which consequently led the security researcher to be more aware of the attack through these popular channels. 

Paul et al. identified some security breaches of wireless insulin pump system and proposed mitigation strategies against the threats \cite{paul2011review}. They were also able to send command from an unauthorized program \cite{paul2010pastpresent}.  Sorber et al. examined the security of mobile health (mHealth) systems in which personal mobile devices serve as a gateway between the EMR management system and medical sensor devices. They proposed an architecture, \emph{Amulet}, that will ensure privacy and security of mHealth system \cite{sorber2012amulet}. Arney et al. described some active and passive attack model on Biomedical devices \cite{arney2011biomedical} over wireless channel. They focused on patient's physical security, clinical data security and privacy, and medical device security. They also identified some key challenges for which the security of the medical devices is still a nightmare. Goodman et al. examined the possibility of homicide and extortion attacks by hacking implantable medical devices \cite{goodman2011does}. He also pointed out the difficulty of investigating this type of homicide cases.

We leverage this body of existing research in exploring the threats to medical devices. The threats from infected mobile devices to medical devices, the core focus of this paper, has not been explored fully by researchers. The closest research related to our work is done by Sorber et al., who proposed a smart card based software security scheme for mobile applications \cite{poster:sorber2012trust}. While their approach allows creating trustworthy applications on mobile devices, they do not consider what will happen if the malware itself is capable of communicating with sensor devices. However, we have already pointed out the strength of the smart devices as a tool for hacking, such as hacking a car's ECU by android phone through the Bluetooth channel \cite{checkoway2011comprehensive}. In this paper, we take the first step in exploring the threats from mobile malware to medical devices. Though no real attack has not been yet recorded, we must explore this new threat model to take some early defenses against real attacker.\\
